Generative Modelling With Inverse Heat Dissipation

While diffusion models have shown great success in image generation, their noise-inverting generative process does not explicitly consider the structure of images, such as their inherent multi-scale nature. Inspired by diffusion models and the empirical success of coarse-to-fine modelling, we propose a new diffusion-like model that generates images through stochastically reversing the heat equation, a PDE that locally erases fine-scale information when run over the 2D plane of the image. We interpret the solution of the forward heat equation with constant additive noise as a variational approximation in the diffusion latent variable model. Our new model shows emergent qualitative properties not seen in standard diffusion models, such as disentanglement of overall colour and shape in images. Spectral analysis on natural images highlights connections to diffusion models and reveals an implicit coarse-to-fine inductive bias in them.

==> fig/psd_diffusion_vs_our.tex <==
% This file was created with tikzplotlib v0.10.1.
\definecolor{blanchedalmond253223209}{RGB}{253,223,209}
\definecolor{cornflowerblue106173213}{RGB}{106,173,213}
\definecolor{crimson2385843}{RGB}{238,58,43}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{firebrick1631420}{RGB}{163,14,20}
\definecolor{firebrick2022328}{RGB}{202,23,28}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lightpink252186160}{RGB}{252,186,160}
\definecolor{lightsteelblue157201224}{RGB}{157,201,224}
\definecolor{maroon103012}{RGB}{103,0,12}
\definecolor{midnightblue848107}{RGB}{8,48,107}
\definecolor{powderblue197218238}{RGB}{197,218,238}
\definecolor{salmon251145113}{RGB}{251,145,113}
\definecolor{steelblue32112180}{RGB}{32,112,180}
\definecolor{steelblue65145197}{RGB}{65,145,197}
\definecolor{teal880154}{RGB}{8,80,154}
\definecolor{tomato25010573}{RGB}{250,105,73}

\begin{axis}[
height=\figureheight,
log basis x={10},
log basis y={10},
tick align=outside,
ytick pos=left,
xtick pos=top,
width=\figurewidth,
x grid style={darkgray176},
xlabel={Frequency},
xmin=0.0118789790974758, xmax=1.8,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Power spectral density},
ymin=5e-05, ymax=100,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, maroon103012]
table {%
0 4232.72802734375
0.0144307506364602 32.3540534973145
0.0288615012729203 5.70585870742798
0.0432922519093805 0.829827964305878
0.0577230025458406 0.559547245502472
0.0721537531823008 0.516008019447327
0.0865845038187609 0.342139214277267
0.101015254455221 0.120390877127647
0.115446005091681 0.0809205174446106
0.129876755728141 0.063157744705677
0.144307506364602 0.0595887713134289
0.158738257001062 0.0413519702851772
0.173169007637522 0.0370372347533703
0.187599758273982 0.0275098532438278
0.202030508910442 0.0312820337712765
0.216461259546902 0.0234983172267675
0.230892010183362 0.0228296052664518
0.245322760819823 0.0146511867642403
0.259753511456283 0.0190396625548601
0.274184262092743 0.0177479963749647
0.288615012729203 0.0162348169833422
0.303045763365663 0.0152454981580377
0.317476514002123 0.0147190941497684
0.331907264638584 0.0151572190225124
0.346338015275044 0.0159449707716703
0.360768765911504 0.0136251309886575
0.375199516547964 0.0122373187914491
0.389630267184424 0.0134431086480618
0.404061017820884 0.0116284796968102
0.418491768457344 0.0131705747917295
0.432922519093805 0.0129350507631898
0.447353269730265 0.0129998475313187
0.461784020366725 0.0113770943135023
0.476214771003185 0.0119259199127555
0.490645521639645 0.0113504668697715
0.505076272276105 0.0121215591207147
0.519507022912566 0.011434025131166
0.533937773549026 0.0110176475718617
0.548368524185486 0.0115459207445383
0.562799274821946 0.011629312299192
0.577230025458406 0.0108891222625971
0.591660776094866 0.0122359627857804
0.606091526731326 0.0131439492106438
0.620522277367787 0.0114798881113529
0.634953028004247 0.00999247189611197
0.649383778640707 0.0112469214946032
0.663814529277167 0.00971411820501089
0.678245279913627 0.00833339337259531
0.692676030550087 0.0197212938219309
0.707106781186548 0.0263331532478333
};
\addplot [semithick, midnightblue848107]
table {%
0 4232.595703125
0.0144307506364602 32.1461601257324
0.0288615012729203 5.65971612930298
0.0432922519093805 0.813514232635498
0.0577230025458406 0.560526728630066
0.0721537531823008 0.487702548503876
0.0865845038187609 0.32972925901413
0.101015254455221 0.103125214576721
0.115446005091681 0.0678141191601753
0.129876755728141 0.0509323254227638
0.144307506364602 0.0468744374811649
0.158738257001062 0.0286952909082174
0.173169007637522 0.0244293380528688
0.187599758273982 0.0157638806849718
0.202030508910442 0.017439890652895
0.216461259546902 0.0134355379268527
0.230892010183362 0.0122982207685709
0.245322760819823 0.00578752066940069
0.259753511456283 0.00834258459508419
0.274184262092743 0.00773796904832125
0.288615012729203 0.00679523823782802
0.303045763365663 0.00559519603848457
0.317476514002123 0.00475169252604246
0.331907264638584 0.00471245963126421
0.346338015275044 0.00484595494344831
0.360768765911504 0.00329058105126023
0.375199516547964 0.00276206620037556
0.389630267184424 0.00296862819232047
0.404061017820884 0.00219366024248302
0.418491768457344 0.00239231018349528
0.432922519093805 0.00229153456166387
0.447353269730265 0.0020539874676615
0.461784020366725 0.00207337667234242
0.476214771003185 0.00182365975342691
0.490645521639645 0.00173470645677298
0.505076272276105 0.00194561725948006
0.519507022912566 0.00128367973957211
0.533937773549026 0.0013019701000303
0.548368524185486 0.00137799617368728
0.562799274821946 0.00144244555849582
0.577230025458406 0.00153251539450139
0.591660776094866 0.00116189639084041
0.606091526731326 0.00147455034311861
0.620522277367787 0.00107528606895357
0.634953028004247 0.00111735088285059
0.649383778640707 0.00103423290420324
0.663814529277167 0.000871932134032249
0.678245279913627 0.000899988459423184
0.692676030550087 0.000545509916264564
0.707106781186548 0.000447459111455828
};
\addplot [semithick, firebrick1631420]
table {%
0 4223.55615234375
0.0144307506364602 32.1678237915039
0.0288615012729203 5.73365783691406
0.0432922519093805 0.989557802677155
0.0577230025458406 0.792178928852081
0.0721537531823008 0.637542307376862
0.0865845038187609 0.464659005403519
0.101015254455221 0.203098118305206
0.115446005091681 0.265425860881805
0.129876755728141 0.201918840408325
0.144307506364602 0.218728765845299
0.158738257001062 0.147750124335289
0.173169007637522 0.170759707689285
0.187599758273982 0.142209827899933
0.202030508910442 0.200928300619125
0.216461259546902 0.16546656191349
0.230892010183362 0.145705133676529
0.245322760819823 0.150196194648743
0.259753511456283 0.175694853067398
0.274184262092743 0.135331809520721
0.288615012729203 0.155511200428009
0.303045763365663 0.135101020336151
0.317476514002123 0.157389998435974
0.331907264638584 0.155329778790474
0.346338015275044 0.15796422958374
0.360768765911504 0.155798673629761
0.375199516547964 0.1356181204319
0.389630267184424 0.142154440283775
0.404061017820884 0.174556896090508
0.418491768457344 0.146739080548286
0.432922519093805 0.150987714529037
0.447353269730265 0.148271441459656
0.461784020366725 0.149650886654854
0.476214771003185 0.143534764647484
0.490645521639645 0.146082267165184
0.505076272276105 0.153857499361038
0.519507022912566 0.14751410484314
0.533937773549026 0.158328637480736
0.548368524185486 0.145813196897507
0.562799274821946 0.163104087114334
0.577230025458406 0.164729967713356
0.591660776094866 0.150858163833618
0.606091526731326 0.151792004704475
0.620522277367787 0.121777035295963
0.634953028004247 0.131536975502968
0.649383778640707 0.148479446768761
0.663814529277167 0.153773665428162
0.678245279913627 0.115268371999264
0.692676030550087 0.192342907190323
0.707106781186548 0.301625788211823
};
\addplot [semithick, teal880154]
table {%
0 4232.595703125
0.0144307506364602 32.1147117614746
0.0288615012729203 5.63547134399414
0.0432922519093805 0.80489844083786
0.0577230025458406 0.549961507320404
0.0721537531823008 0.473232239484787
0.0865845038187609 0.316132217645645
0.101015254455221 0.0972629487514496
0.115446005091681 0.0628609880805016
0.129876755728141 0.0461945682764053
0.144307506364602 0.0415583923459053
0.158738257001062 0.0248176325112581
0.173169007637522 0.0204616114497185
0.187599758273982 0.0128250624984503
0.202030508910442 0.0136999050155282
0.216461259546902 0.0102091198787093
0.230892010183362 0.00898506212979555
0.245322760819823 0.00399197963997722
0.259753511456283 0.00555962650105357
0.274184262092743 0.00489618768915534
0.288615012729203 0.00409731734544039
0.303045763365663 0.00319936405867338
0.317476514002123 0.0025296148378402
0.331907264638584 0.00238723400980234
0.346338015275044 0.0023198421113193
0.360768765911504 0.00143199763260782
0.375199516547964 0.00111098773777485
0.389630267184424 0.00114385015331209
0.404061017820884 0.000754182517994195
0.418491768457344 0.00077186751877889
0.432922519093805 0.000663120299577713
0.447353269730265 0.000551210134290159
0.461784020366725 0.000520520203281194
0.476214771003185 0.000427464110543951
0.490645521639645 0.000380304380087182
0.505076272276105 0.000391929381294176
0.519507022912566 0.000217399283428676
0.533937773549026 0.000209745281608775
0.548368524185486 0.000200941372895613
0.562799274821946 0.000183484953595325
0.577230025458406 0.000179907452547923
0.591660776094866 0.000109025866549928
0.606091526731326 0.000133702880702913
0.620522277367787 8.60300206113607e-05
0.634953028004247 8.86320558493026e-05
0.649383778640707 7.17630682629533e-05
0.663814529277167 5.78750514250714e-05
0.678245279913627 5.40353539690841e-05
0.692676030550087 3.10114482999779e-05
0.707106781186548 2.77639446721878e-05
};
\addplot [semithick, firebrick2022328]
table {%
0 4061.59497070312
0.0144307506364602 30.1168060302734
0.0288615012729203 6.88720369338989
0.0432922519093805 1.42177736759186
0.0577230025458406 1.23456656932831
0.0721537531823008 1.27215051651001
0.0865845038187609 1.06069076061249
0.101015254455221 0.806882441043854
0.115446005091681 0.847575664520264
0.129876755728141 0.866420328617096
0.144307506364602 0.840149939060211
0.158738257001062 0.829099893569946
0.173169007637522 0.725609660148621
0.187599758273982 0.843374967575073
0.202030508910442 0.768321812152863
0.216461259546902 0.813376843929291
0.230892010183362 0.70635986328125
0.245322760819823 0.801679730415344
0.259753511456283 0.780491292476654
0.274184262092743 0.782661259174347
0.288615012729203 0.806313037872314
0.303045763365663 0.808813452720642
0.317476514002123 0.732280850410461
0.331907264638584 0.788961410522461
0.346338015275044 0.777129471302032
0.360768765911504 0.732400596141815
0.375199516547964 0.800196647644043
0.389630267184424 0.69126969575882
0.404061017820884 0.754157602787018
0.418491768457344 0.806262969970703
0.432922519093805 0.71738201379776
0.447353269730265 0.728827774524689
0.461784020366725 0.748048961162567
0.476214771003185 0.660145699977875
0.490645521639645 0.671835064888
0.505076272276105 0.73305606842041
0.519507022912566 0.755277574062347
0.533937773549026 0.844465970993042
0.548368524185486 0.793608248233795
0.562799274821946 0.713270366191864
0.577230025458406 0.72947758436203
0.591660776094866 0.752604365348816
0.606091526731326 0.646145343780518
0.620522277367787 0.816494345664978
0.634953028004247 0.778536677360535
0.649383778640707 0.894367814064026
0.663814529277167 0.817768394947052
0.678245279913627 0.72534853219986
0.692676030550087 0.645110726356506
0.707106781186548 0.890538036823273
};
\addplot [semithick, steelblue32112180]
table {%
0 4232.595703125
0.0144307506364602 32.012020111084
0.0288615012729203 5.55692625045776
0.0432922519093805 0.777480661869049
0.0577230025458406 0.516841888427734
0.0721537531823008 0.428886771202087
0.0865845038187609 0.275526493787766
0.101015254455221 0.0804435908794403
0.115446005091681 0.0492292866110802
0.129876755728141 0.0337259247899055
0.144307506364602 0.0281904395669699
0.158738257001062 0.0156179750338197
0.173169007637522 0.01165188010782
0.187599758273982 0.00666680373251438
0.202030508910442 0.00641467003151774
0.216461259546902 0.00430490309372544
0.230892010183362 0.0033513936214149
0.245322760819823 0.00131047912873328
0.259753511456283 0.00158182089217007
0.274184262092743 0.00121556222438812
0.288615012729203 0.000874013465363532
0.303045763365663 0.000586095731705427
0.317476514002123 0.000390782282920554
0.331907264638584 0.000309942697640508
0.346338015275044 0.000252380355959758
0.360768765911504 0.000126676328363828
0.375199516547964 8.03585353423841e-05
0.389630267184424 6.77298521623015e-05
0.404061017820884 3.54096555383876e-05
0.418491768457344 2.89329600491328e-05
0.432922519093805 1.88360463653225e-05
0.447353269730265 1.20564336612006e-05
0.461784020366725 8.68760525918333e-06
0.476214771003185 5.59583668291452e-06
0.490645521639645 3.77815626961819e-06
0.505076272276105 3.08917196889524e-06
0.519507022912566 1.24511325338972e-06
0.533937773549026 9.33093929234019e-07
0.548368524185486 6.56987765523809e-07
0.562799274821946 4.1528520000611e-07
0.577230025458406 3.14052471139803e-07
0.591660776094866 1.23462243095673e-07
0.606091526731326 1.08259889941564e-07
0.620522277367787 4.9725194628536e-08
0.634953028004247 3.68927040028666e-08
0.649383778640707 2.01463095095278e-08
0.663814529277167 1.16870140232095e-08
0.678245279913627 6.45820374955974e-09
0.692676030550087 2.66648059188412e-09
0.707106781186548 3.04381897464623e-09
};
\addplot [semithick, crimson2385843]
table {%
0 4054.27416992188
0.0144307506364602 34.4068717956543
0.0288615012729203 7.82698631286621
0.0432922519093805 3.85997366905212
0.0577230025458406 2.44678258895874
0.0721537531823008 2.60799503326416
0.0865845038187609 3.05884909629822
0.101015254455221 2.11519169807434
0.115446005091681 2.32988619804382
0.129876755728141 2.39462447166443
0.144307506364602 2.6806640625
0.158738257001062 2.14962887763977
0.173169007637522 2.7410740852356
0.187599758273982 2.45903730392456
0.202030508910442 2.57933449745178
0.216461259546902 2.33689665794373
0.230892010183362 2.29256963729858
0.245322760819823 2.42338418960571
0.259753511456283 2.34181833267212
0.274184262092743 2.53146982192993
0.288615012729203 2.11029839515686
0.303045763365663 2.33430337905884
0.317476514002123 2.35655570030212
0.331907264638584 2.31299233436584
0.346338015275044 2.56668972969055
0.360768765911504 2.46497678756714
0.375199516547964 2.34936833381653
0.389630267184424 2.37999701499939
0.404061017820884 2.38169074058533
0.418491768457344 2.21555638313293
0.432922519093805 2.28267884254456
0.447353269730265 2.61344194412231
0.461784020366725 2.31768107414246
0.476214771003185 2.33294153213501
0.490645521639645 2.22459745407104
0.505076272276105 2.40822315216064
0.519507022912566 2.26807713508606
0.533937773549026 2.38190078735352
0.548368524185486 2.49763751029968
0.562799274821946 2.74748969078064
0.577230025458406 2.61627221107483
0.591660776094866 2.39180159568787
0.606091526731326 2.94460082054138
0.620522277367787 2.31383323669434
0.634953028004247 2.25491833686829
0.649383778640707 2.23260164260864
0.663814529277167 2.32771182060242
0.678245279913627 2.49445557594299
0.692676030550087 2.12927961349487
0.707106781186548 3.24970960617065
};
\addplot [semithick, steelblue65145197]
table {%
0 4232.595703125
0.0144307506364602 31.6779670715332
0.0288615012729203 5.30787515640259
0.0432922519093805 0.694169998168945
0.0577230025458406 0.421692788600922
0.0721537531823008 0.310798048973083
0.0865845038187609 0.175667479634285
0.101015254455221 0.0431997030973434
0.115446005091681 0.02213229611516
0.129876755728141 0.0120455268770456
0.144307506364602 0.00790988374501467
0.158738257001062 0.00343049457296729
0.173169007637522 0.00184532231651247
0.187599758273982 0.000782591523602605
0.202030508910442 0.000534665305167437
0.216461259546902 0.000255766994087026
0.230892010183362 0.000133065113914199
0.245322760819823 3.43588035320863e-05
0.259753511456283 2.59480020758929e-05
0.274184262092743 1.27556104416726e-05
0.288615012729203 5.62550985705457e-06
0.303045763365663 2.29044280786184e-06
0.317476514002123 8.83128677742206e-07
0.331907264638584 3.97489543502161e-07
0.346338015275044 1.83016084065457e-07
0.360768765911504 4.7961709270794e-08
0.375199516547964 1.62408557713434e-08
0.389630267184424 7.03585989469957e-09
0.404061017820884 1.85701687360762e-09
0.418491768457344 7.49651674070151e-10
0.432922519093805 2.22748333666978e-10
0.447353269730265 6.55991927445143e-11
0.461784020366725 2.13660495546053e-11
0.476214771003185 6.10683855914451e-12
0.490645521639645 1.56293066596452e-12
0.505076272276105 6.46813711532163e-13
0.519507022912566 9.83415958258696e-14
0.533937773549026 3.47917631119896e-14
0.548368524185486 1.23612845830058e-14
0.562799274821946 5.82429891872482e-15
0.577230025458406 3.5464587640015e-15
0.591660776094866 5.13178934500517e-15
0.606091526731326 6.89166080566949e-15
0.620522277367787 3.99667371612611e-15
0.634953028004247 4.45789924953207e-15
0.649383778640707 4.70220345679447e-15
0.663814529277167 6.38970781057717e-15
0.678245279913627 1.17507432346249e-14
0.692676030550087 1.45377874099855e-14
0.707106781186548 4.20058952899094e-14
};
\addplot [semithick, tomato25010573]
table {%
0 4891.0947265625
0.0144307506364602 42.6237564086914
0.0288615012729203 8.75174617767334
0.0432922519093805 6.778000831604
0.0577230025458406 5.53348541259766
0.0721537531823008 5.8361382484436
0.0865845038187609 6.48051118850708
0.101015254455221 5.44920253753662
0.115446005091681 6.38760757446289
0.129876755728141 6.01622343063354
0.144307506364602 5.48472452163696
0.158738257001062 5.88302326202393
0.173169007637522 5.67763471603394
0.187599758273982 5.83057403564453
0.202030508910442 5.92439079284668
0.216461259546902 6.37825727462769
0.230892010183362 5.4368724822998
0.245322760819823 5.83675909042358
0.259753511456283 5.27672386169434
0.274184262092743 5.90139245986938
0.288615012729203 6.14822101593018
0.303045763365663 6.52053356170654
0.317476514002123 6.38525390625
0.331907264638584 5.84659671783447
0.346338015275044 5.27956056594849
0.360768765911504 6.22186231613159
0.375199516547964 5.718337059021
0.389630267184424 6.0346417427063
0.404061017820884 6.89417934417725
0.418491768457344 5.77531480789185
0.432922519093805 5.81436681747437
0.447353269730265 5.91966390609741
0.461784020366725 5.95116853713989
0.476214771003185 5.8105149269104
0.490645521639645 6.14352512359619
0.505076272276105 5.99803113937378
0.519507022912566 6.55780029296875
0.533937773549026 6.08819150924683
0.548368524185486 6.25752401351929
0.562799274821946 5.29213047027588
0.577230025458406 6.11114931106567
0.591660776094866 6.26348447799683
0.606091526731326 5.60617208480835
0.620522277367787 5.15372657775879
0.634953028004247 5.78413724899292
0.649383778640707 5.9236307144165
0.663814529277167 4.88249731063843
0.678245279913627 6.96924686431885
0.692676030550087 3.27663683891296
0.707106781186548 9.06750297546387
};
\addplot [semithick, cornflowerblue106173213]
table {%
0 4232.5966796875
0.0144307506364602 30.6125526428223
0.0288615012729203 4.57623720169067
0.0432922519093805 0.480485081672668
0.0577230025458406 0.217083498835564
0.0721537531823008 0.108974128961563
0.0865845038187609 0.0405610427260399
0.101015254455221 0.00569701800122857
0.115446005091681 0.00165058020502329
0.129876755728141 0.000422577693825588
0.144307506364602 0.000125633712741546
0.158738257001062 2.46755007538013e-05
0.173169007637522 4.57584428659175e-06
0.187599758273982 7.25009726920689e-07
0.202030508910442 1.61459567493694e-07
0.216461259546902 2.65529997989233e-08
0.230892010183362 3.64887253745394e-09
0.245322760819823 2.44158387951998e-10
0.259753511456283 4.02758174034012e-11
0.274184262092743 4.45142880889371e-12
0.288615012729203 4.17667853427894e-13
0.303045763365663 4.04720270426491e-14
0.317476514002123 1.12135845856294e-14
0.331907264638584 6.34215580443478e-15
0.346338015275044 4.03838966526191e-15
0.360768765911504 4.16832282530482e-15
0.375199516547964 8.72182541304407e-15
0.389630267184424 4.91154214399422e-15
0.404061017820884 4.15945693144591e-15
0.418491768457344 4.56785301993163e-15
0.432922519093805 6.71768023830345e-15
0.447353269730265 7.05268092190958e-15
0.461784020366725 3.93523502832996e-15
0.476214771003185 3.18146654955723e-15
0.490645521639645 5.67156532580771e-15
0.505076272276105 4.61891047192622e-15
0.519507022912566 3.51809036004853e-15
0.533937773549026 3.53771039596402e-15
0.548368524185486 3.45453472515897e-15
0.562799274821946 3.73017978674449e-15
0.577230025458406 2.96096905031036e-15
0.591660776094866 3.36603947568691e-15
0.606091526731326 3.23451495249435e-15
0.620522277367787 3.76517622350972e-15
0.634953028004247 2.52712957439678e-15
0.649383778640707 3.2479184018517e-15
0.663814529277167 3.25788755612441e-15
0.678245279913627 4.2473501522507e-15
0.692676030550087 5.63145153949164e-15
0.707106781186548 2.49099896051518e-15
};
\addplot [semithick, salmon251145113]
table {%
0 3719.2265625
0.0144307506364602 34.6678161621094
0.0288615012729203 21.2172031402588
0.0432922519093805 14.2057113647461
0.0577230025458406 14.8072490692139
0.0721537531823008 10.6460428237915
0.0865845038187609 14.7996597290039
0.101015254455221 11.215368270874
0.115446005091681 11.5155744552612
0.129876755728141 10.3095760345459
0.144307506364602 13.4900341033936
0.158738257001062 13.0478515625
0.173169007637522 12.003321647644
0.187599758273982 11.9335021972656
0.202030508910442 12.2246255874634
0.216461259546902 11.1818113327026
0.230892010183362 13.1375064849854
0.245322760819823 11.2792692184448
0.259753511456283 14.6660861968994
0.274184262092743 12.4957504272461
0.288615012729203 12.4463529586792
0.303045763365663 11.5226650238037
0.317476514002123 11.4964723587036
0.331907264638584 12.5897150039673
0.346338015275044 10.8554067611694
0.360768765911504 10.7297630310059
0.375199516547964 11.9784536361694
0.389630267184424 11.6116943359375
0.404061017820884 13.5273723602295
0.418491768457344 13.3186950683594
0.432922519093805 11.7902050018311
0.447353269730265 11.6081743240356
0.461784020366725 11.4796895980835
0.476214771003185 12.5856904983521
0.490645521639645 11.4915628433228
0.505076272276105 11.7020893096924
0.519507022912566 11.5543727874756
0.533937773549026 11.3106422424316
0.548368524185486 11.6612548828125
0.562799274821946 13.1983289718628
0.577230025458406 10.8495388031006
0.591660776094866 11.888035774231
0.606091526731326 11.6846313476562
0.620522277367787 11.0017318725586
0.634953028004247 12.3904590606689
0.649383778640707 12.7875127792358
0.663814529277167 10.2114515304565
0.678245279913627 9.77107238769531
0.692676030550087 14.0592212677002
0.707106781186548 15.327374458313
};
\addplot [semithick, lightsteelblue157201224]
table {%
0 4232.5966796875
0.0144307506364602 27.4243202209473
0.0288615012729203 2.87464022636414
0.0432922519093805 0.149445429444313
0.0577230025458406 0.0254597496241331
0.0721537531823008 0.00383229507133365
0.0865845038187609 0.000373971532098949
0.101015254455221 8.73476983542787e-06
0.115446005091681 4.25435018769349e-07
0.129876755728141 9.28846421999197e-09
0.144307506364602 2.0665018307664e-10
0.158738257001062 3.25755156356522e-12
0.173169007637522 2.50118563284874e-14
0.187599758273982 1.0845780010042e-14
0.202030508910442 4.73311507717157e-15
0.216461259546902 3.0287558265297e-15
0.230892010183362 3.76700115599458e-15
0.245322760819823 1.37306056688337e-14
0.259753511456283 5.41936550092748e-15
0.274184262092743 5.15261322649695e-15
0.288615012729203 3.65379181446225e-15
0.303045763365663 4.27515993797496e-15
0.317476514002123 1.15975751138059e-14
0.331907264638584 5.17430743434202e-15
0.346338015275044 4.34892846086781e-15
0.360768765911504 3.39886179063478e-15
0.375199516547964 1.06066371980437e-14
0.389630267184424 4.34366584516651e-15
0.404061017820884 3.18325484786712e-15
0.418491768457344 2.91599287136058e-15
0.432922519093805 8.31383505334009e-15
0.447353269730265 4.46427698410842e-15
0.461784020366725 3.96807703679385e-15
0.476214771003185 2.93136016660614e-15
0.490645521639645 6.18601078632261e-15
0.505076272276105 1.47112207940676e-14
0.519507022912566 3.33620909286699e-15
0.533937773549026 3.08440673819725e-15
0.548368524185486 3.08116726069048e-15
0.562799274821946 3.01278883195748e-15
0.577230025458406 2.71319878422779e-15
0.591660776094866 2.7115542697607e-15
0.606091526731326 3.78964742887237e-15
0.620522277367787 4.44431284105811e-15
0.634953028004247 3.30294420320418e-15
0.649383778640707 4.8244201466879e-15
0.663814529277167 5.62022157667695e-15
0.678245279913627 3.365969807227e-15
0.692676030550087 4.7561814783912e-15
0.707106781186548 6.77419004137952e-15
};
\addplot [semithick, lightpink252186160]
table {%
0 3397.36840820312
0.0144307506364602 80.3670501708984
0.0288615012729203 32.544116973877
0.0432922519093805 24.9172668457031
0.0577230025458406 21.8859615325928
0.0721537531823008 21.0322227478027
0.0865845038187609 21.8993988037109
0.101015254455221 25.698221206665
0.115446005091681 23.3525257110596
0.129876755728141 19.8684768676758
0.144307506364602 22.504150390625
0.158738257001062 21.6451835632324
0.173169007637522 22.7815914154053
0.187599758273982 25.4074172973633
0.202030508910442 20.7947692871094
0.216461259546902 21.6104736328125
0.230892010183362 21.0608215332031
0.245322760819823 23.758810043335
0.259753511456283 24.2590408325195
0.274184262092743 22.9093208312988
0.288615012729203 21.7586154937744
0.303045763365663 22.605842590332
0.317476514002123 21.9528064727783
0.331907264638584 22.3961391448975
0.346338015275044 22.1113433837891
0.360768765911504 22.0110454559326
0.375199516547964 21.5510292053223
0.389630267184424 24.2211170196533
0.404061017820884 21.6260261535645
0.418491768457344 24.6530418395996
0.432922519093805 22.7725391387939
0.447353269730265 23.5202598571777
0.461784020366725 23.2158317565918
0.476214771003185 21.384464263916
0.490645521639645 20.8208866119385
0.505076272276105 22.4905776977539
0.519507022912566 24.0605964660645
0.533937773549026 20.7480411529541
0.548368524185486 23.3599662780762
0.562799274821946 23.5281429290771
0.577230025458406 18.9159469604492
0.591660776094866 22.7341003417969
0.606091526731326 22.1532135009766
0.620522277367787 21.5853519439697
0.634953028004247 22.5922946929932
0.649383778640707 25.4843769073486
0.663814529277167 18.3918571472168
0.678245279913627 23.9442081451416
0.692676030550087 20.043643951416
0.707106781186548 14.6131362915039
};
\addplot [semithick, powderblue197218238]
table {%
0 4232.595703125
0.0144307506364602 19.5961399078369
0.0288615012729203 0.746747314929962
0.0432922519093805 0.00429745810106397
0.0577230025458406 2.97548158414429e-05
0.0721537531823008 1.37171355163446e-07
0.0865845038187609 2.22217355627663e-10
0.101015254455221 2.21517716550521e-14
0.115446005091681 6.29273312602839e-15
0.129876755728141 2.12868984998628e-14
0.144307506364602 6.25069064569142e-15
0.158738257001062 9.03656337448598e-15
0.173169007637522 5.92154634788261e-15
0.187599758273982 6.04418062501904e-15
0.202030508910442 6.78444210465662e-15
0.216461259546902 3.85327400277127e-15
0.230892010183362 4.68051094301529e-15
0.245322760819823 2.37894420959325e-14
0.259753511456283 5.94322361506874e-15
0.274184262092743 3.71341785175127e-15
0.288615012729203 2.74063460490583e-15
0.303045763365663 3.67275899973364e-15
0.317476514002123 4.73228329081737e-15
0.331907264638584 2.5527607913807e-15
0.346338015275044 3.45052360063724e-15
0.360768765911504 4.33509895393798e-15
0.375199516547964 3.15547237895542e-15
0.389630267184424 2.49879822813526e-15
0.404061017820884 4.3887944900468e-15
0.418491768457344 2.64462024396101e-15
0.432922519093805 6.64689454193436e-15
0.447353269730265 4.15765359830121e-15
0.461784020366725 6.17626101358324e-15
0.476214771003185 2.34027050634246e-15
0.490645521639645 3.81896154511095e-15
0.505076272276105 2.93216633021369e-15
0.519507022912566 2.5809384011623e-15
0.533937773549026 3.28592159382145e-15
0.548368524185486 1.70749824886528e-15
0.562799274821946 2.13382994237175e-15
0.577230025458406 2.12253136988832e-15
0.591660776094866 2.61080859453075e-15
0.606091526731326 2.08868329804133e-15
0.620522277367787 2.67841897613882e-15
0.634953028004247 2.87378373729124e-15
0.649383778640707 3.34871871070675e-15
0.663814529277167 1.69402661335567e-15
0.678245279913627 3.39192797892856e-15
0.692676030550087 7.04556923328443e-15
0.707106781186548 1.18704806590817e-14
};
\addplot [semithick, blanchedalmond253223209]
table {%
0 5553.5166015625
0.0144307506364602 44.327507019043
0.0288615012729203 32.1998596191406
0.0432922519093805 34.6094512939453
0.0577230025458406 40.8034477233887
0.0721537531823008 41.0219955444336
0.0865845038187609 37.7894439697266
0.101015254455221 40.4048614501953
0.115446005091681 37.4674797058105
0.129876755728141 42.6233291625977
0.144307506364602 46.9966278076172
0.158738257001062 37.3209457397461
0.173169007637522 40.1695404052734
0.187599758273982 31.9853763580322
0.202030508910442 42.5834617614746
0.216461259546902 44.7080879211426
0.230892010183362 43.8096961975098
0.245322760819823 38.3715438842773
0.259753511456283 39.9169158935547
0.274184262092743 39.7386932373047
0.288615012729203 41.0588874816895
0.303045763365663 40.1328544616699
0.317476514002123 39.9809150695801
0.331907264638584 39.9396438598633
0.346338015275044 36.2324028015137
0.360768765911504 41.861515045166
0.375199516547964 38.4459533691406
0.389630267184424 37.3663558959961
0.404061017820884 38.6298294067383
0.418491768457344 37.2620582580566
0.432922519093805 36.7837142944336
0.447353269730265 35.9628448486328
0.461784020366725 41.6815452575684
0.476214771003185 35.7786712646484
0.490645521639645 35.8205108642578
0.505076272276105 40.0615882873535
0.519507022912566 41.3818511962891
0.533937773549026 40.6462631225586
0.548368524185486 46.2661476135254
0.562799274821946 46.8507347106934
0.577230025458406 38.3078994750977
0.591660776094866 48.7730102539062
0.606091526731326 38.5891609191895
0.620522277367787 36.2998695373535
0.634953028004247 38.9881362915039
0.649383778640707 33.8608360290527
0.663814529277167 44.037841796875
0.678245279913627 30.0820026397705
0.692676030550087 23.1101875305176
0.707106781186548 57.9885444641113
};
\addplot [semithick, lavender221234246]
table {%
0 4232.595703125
0.0144307506364602 8.31308460235596
0.0288615012729203 0.0173466373234987
0.0432922519093805 7.93604755244814e-08
0.0577230025458406 6.88838702332835e-14
0.0721537531823008 8.40356040640979e-15
0.0865845038187609 2.07742148678781e-14
0.101015254455221 6.92309716295741e-15
0.115446005091681 1.20853398835152e-14
0.129876755728141 6.33945207526715e-14
0.144307506364602 2.92895353424475e-15
0.158738257001062 3.62276584463727e-15
0.173169007637522 4.79427424409512e-15
0.187599758273982 2.673000294617e-15
0.202030508910442 8.65700367565659e-15
0.216461259546902 5.74831879280669e-15
0.230892010183362 7.6149380041652e-15
0.245322760819823 5.23802836771125e-14
0.259753511456283 3.89746752327779e-15
0.274184262092743 4.90594876192702e-15
0.288615012729203 2.28524978718766e-15
0.303045763365663 2.95064710681512e-15
0.317476514002123 1.53479845884296e-14
0.331907264638584 4.70872222235654e-15
0.346338015275044 5.20838526387596e-15
0.360768765911504 3.13397362396292e-15
0.375199516547964 4.06460152333117e-15
0.389630267184424 3.02813685720349e-15
0.404061017820884 4.63905376244488e-15
0.418491768457344 3.56479829785898e-15
0.432922519093805 4.22278746732975e-15
0.447353269730265 1.909243391572e-15
0.461784020366725 2.90449651668397e-15
0.476214771003185 1.91814782543002e-15
0.490645521639645 2.86605540868049e-15
0.505076272276105 1.46631889437606e-14
0.519507022912566 2.20381095744095e-15
0.533937773549026 1.67189205425714e-15
0.548368524185486 2.11890225722581e-15
0.562799274821946 1.41349988913689e-15
0.577230025458406 1.46772069155212e-15
0.591660776094866 1.95939176545596e-15
0.606091526731326 1.86600871236178e-15
0.620522277367787 2.35505377237089e-15
0.634953028004247 2.02329934253511e-15
0.649383778640707 1.84437231451535e-15
0.663814529277167 2.07546788999827e-15
0.678245279913627 2.78405986652919e-15
0.692676030550087 1.58461176766881e-15
0.707106781186548 4.35921186436395e-15
};
\addplot [thick, black]
table {%
0 4232.595703125
0.0144307506364602 32.1605834960938
0.0288615012729203 5.6709418296814
0.0432922519093805 0.817931830883026
0.0577230025458406 0.56571888923645
0.0721537531823008 0.494699031114578
0.0865845038187609 0.336380869150162
0.101015254455221 0.106302551925182
0.115446005091681 0.070722334086895
0.129876755728141 0.0537596493959427
0.144307506364602 0.0500278733670712
0.158738257001062 0.031267873942852
0.173169007637522 0.0271262433379889
0.187599758273982 0.0178658775985241
0.202030508910442 0.0202178955078125
0.216461259546902 0.0158419366925955
0.230892010183362 0.0147985853254795
0.245322760819823 0.00752361165359616
0.259753511456283 0.0106848310679197
0.274184262092743 0.0103128561750054
0.288615012729203 0.00923687033355236
0.303045763365663 0.00785864051431417
0.317476514002123 0.00713249342516065
0.331907264638584 0.00709398090839386
0.346338015275044 0.00746010709553957
0.360768765911504 0.00547286495566368
0.375199516547964 0.00477837212383747
0.389630267184424 0.00514542916789651
0.404061017820884 0.00416117906570435
0.418491768457344 0.00458281440660357
0.432922519093805 0.00463917152956128
0.447353269730265 0.00428481865674257
0.461784020366725 0.00440013688057661
0.476214771003185 0.00402449257671833
0.490645521639645 0.00392644666135311
0.505076272276105 0.00450014462694526
0.519507022912566 0.003355034859851
0.533937773549026 0.00338396313600242
0.548368524185486 0.00368841853924096
0.562799274821946 0.00406561559066176
0.577230025458406 0.00440886104479432
0.591660776094866 0.00370914000086486
0.606091526731326 0.00465241866186261
0.620522277367787 0.00355534651316702
0.634953028004247 0.00356505438685417
0.649383778640707 0.00347964628599584
0.663814529277167 0.0029361757915467
0.678245279913627 0.0031173590105027
0.692676030550087 0.00192094186786562
0.707106781186548 0.00151352933607996
};
\end{axis}




==> fig/psd_diffusion_vs_our_new.tex <==
\definecolor{cornflowerblue106173213}{RGB}{106,173,213}
\definecolor{crimson2385843}{RGB}{238,58,43}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{firebrick1631420}{RGB}{163,14,20}
\definecolor{firebrick2022328}{RGB}{202,23,28}
\definecolor{lavender221234246}{RGB}{221,234,246}
\definecolor{lightpink252186160}{RGB}{252,186,160}
\definecolor{lightsteelblue157201224}{RGB}{157,201,224}
\definecolor{maroon103012}{RGB}{103,0,12}
\definecolor{midnightblue848107}{RGB}{8,48,107}
\definecolor{powderblue197218238}{RGB}{197,218,238}
\definecolor{salmon251145113}{RGB}{251,145,113}
\definecolor{steelblue32112180}{RGB}{32,112,180}
\definecolor{steelblue65145197}{RGB}{65,145,197}
\definecolor{teal880154}{RGB}{8,80,154}
\definecolor{tomato25010573}{RGB}{250,105,73}

\begin{axis}[
height=\figureheight,
log basis x={10},
log basis y={10},
tick align=outside,
ytick pos=left,
xtick pos=top,
width=\figurewidth,
x grid style={darkgray176},
xlabel={Frequency},
xmin=0.0746378307121039, xmax=12,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Power spectral density},
ymin=5e-06, ymax=100,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, maroon103012]
table {%
0 1130.20397949219
0.0906710848212242 26.2868309020996
0.181342169642448 1.93730807304382
0.272013247013092 1.12687683105469
0.362684339284897 0.328138262033463
0.453355401754379 0.199038937687874
0.544026494026184 0.0982919782400131
0.634697556495667 0.0763682350516319
0.725368678569794 0.0548633374273777
0.816039741039276 0.0357935205101967
0.906710803508759 0.0377704538404942
0.997381925582886 0.0277561023831367
1.08805298805237 0.02797563187778
1.17872405052185 0.0194927975535393
1.26939511299133 0.0174087714403868
1.36006617546082 0.015076688490808
1.45073735713959 0.0129146603867412
1.54140841960907 0.0124856121838093
1.63207948207855 0.0113549456000328
1.72275054454803 0.0107967648655176
1.81342160701752 0.0095936693251133
1.904092669487 0.00851880852133036
1.99476385116577 0.00929572712630033
2.08543491363525 0.00781553704291582
2.17610597610474 0.00806594360619783
2.26677703857422 0.0072566089220345
2.3574481010437 0.00742571195587516
2.44811916351318 0.00662446254864335
2.53879022598267 0.00613838620483875
2.62946128845215 0.00601120432838798
2.72013235092163 0.00557282380759716
2.81080365180969 0.00564817106351256
2.90147471427917 0.00536603666841984
2.99214577674866 0.00472792563959956
3.08281683921814 0.00532081956043839
3.17348790168762 0.00540129281580448
3.2641589641571 0.00498692272230983
3.35483002662659 0.00511272763833404
3.44550108909607 0.00492569012567401
3.53617215156555 0.00419347686693072
3.62684321403503 0.00483512785285711
3.71751427650452 0.00416009686887264
3.808185338974 0.00445575593039393
3.89885663986206 0.00509354658424854
3.98952770233154 0.00355815095826983
4.08019876480103 0.0040506268851459
4.17086982727051 0.00394955743104219
4.26154088973999 0.0044204113073647
4.35221195220947 0.00191259675193578
4.44288301467896 0.00188842648640275
};
\addplot [semithick, midnightblue848107]
table {%
0 1126.79028320312
0.0906710848212242 25.9501171112061
0.181342169642448 1.93539273738861
0.272013247013092 1.09762954711914
0.362684339284897 0.31594580411911
0.453355401754379 0.170278459787369
0.544026494026184 0.0890136584639549
0.634697556495667 0.0651832669973373
0.725368678569794 0.0434334613382816
0.816039741039276 0.0254299826920033
0.906710803508759 0.0268976595252752
0.997381925582886 0.0190354827791452
1.08805298805237 0.0167999174445868
1.17872405052185 0.010500063188374
1.26939511299133 0.00871535949409008
1.36006617546082 0.00675312848761678
1.45073735713959 0.00562699045985937
1.54140841960907 0.00448392378166318
1.63207948207855 0.00369015568867326
1.72275054454803 0.00318543030880392
1.81342160701752 0.00249320757575333
1.904092669487 0.00200685136951506
1.99476385116577 0.00164494290947914
2.08543491363525 0.00146548543125391
2.17610597610474 0.00117106072138995
2.26677703857422 0.0010555163025856
2.3574481010437 0.000782711082138121
2.44811916351318 0.000603008666075766
2.53879022598267 0.000467090052552521
2.62946128845215 0.00037849711952731
2.72013235092163 0.000305501773254946
2.81080365180969 0.000208691373700276
2.90147471427917 0.000171440042322502
2.99214577674866 0.000142665579915047
3.08281683921814 0.000107329564343672
3.17348790168762 8.61274893395603e-05
3.2641589641571 6.64867402520031e-05
3.35483002662659 4.67802274215501e-05
3.44550108909607 4.24011486757081e-05
3.53617215156555 3.13082382490393e-05
3.62684321403503 1.73604257724946e-05
3.71751427650452 1.34159427034319e-05
3.808185338974 1.05077033367706e-05
3.89885663986206 9.78398566076066e-06
3.98952770233154 6.76228546581115e-06
4.08019876480103 5.06932201460586e-06
4.17086982727051 3.12733277496591e-06
4.26154088973999 3.46665183315054e-06
4.35221195220947 2.24646942115214e-06
4.44288301467896 8.98965765827597e-07
};
\addplot [semithick, firebrick1631420]
table {%
0 1124.29211425781
0.0906710848212242 25.3056373596191
0.181342169642448 2.09840250015259
0.272013247013092 1.11246824264526
0.362684339284897 0.364209353923798
0.453355401754379 0.228792458772659
0.544026494026184 0.140264287590981
0.634697556495667 0.11166112869978
0.725368678569794 0.0728388205170631
0.816039741039276 0.0698860213160515
0.906710803508759 0.0921328067779541
0.997381925582886 0.0843527987599373
1.08805298805237 0.073869101703167
1.17872405052185 0.0609612055122852
1.26939511299133 0.0675989240407944
1.36006617546082 0.0587482862174511
1.45073735713959 0.0552521608769894
1.54140841960907 0.0546007640659809
1.63207948207855 0.0520252138376236
1.72275054454803 0.056580975651741
1.81342160701752 0.0610514096915722
1.904092669487 0.0510770902037621
1.99476385116577 0.0528083592653275
2.08543491363525 0.0571277365088463
2.17610597610474 0.0473947934806347
2.26677703857422 0.0525504909455776
2.3574481010437 0.0519294366240501
2.44811916351318 0.0546491853892803
2.53879022598267 0.0467904433608055
2.62946128845215 0.0464669652283192
2.72013235092163 0.0466416999697685
2.81080365180969 0.0518748387694359
2.90147471427917 0.0485914349555969
2.99214577674866 0.0451896339654922
3.08281683921814 0.0460189692676067
3.17348790168762 0.0490201786160469
3.2641589641571 0.0495661422610283
3.35483002662659 0.0477956533432007
3.44550108909607 0.0471134781837463
3.53617215156555 0.0445204228162766
3.62684321403503 0.0408992357552052
3.71751427650452 0.0507768094539642
3.808185338974 0.0540976338088512
3.89885663986206 0.0551993362605572
3.98952770233154 0.0447353720664978
4.08019876480103 0.0551976338028908
4.17086982727051 0.0342685058712959
4.26154088973999 0.0529236830770969
4.35221195220947 0.0618366077542305
4.44288301467896 0.00990117620676756
};
\addplot [semithick, teal880154]
table {%
0 1126.7626953125
0.0906710848212242 25.8737602233887
0.181342169642448 1.89835512638092
0.272013247013092 1.05642986297607
0.362684339284897 0.294349044561386
0.453355401754379 0.151720106601715
0.544026494026184 0.075493335723877
0.634697556495667 0.0519290268421173
0.725368678569794 0.0323435105383396
0.816039741039276 0.0174486059695482
0.906710803508759 0.0170393381267786
0.997381925582886 0.0109339449554682
1.08805298805237 0.00868513528257608
1.17872405052185 0.00482944399118423
1.26939511299133 0.00353790610097349
1.36006617546082 0.00239345617592335
1.45073735713959 0.00172698008827865
1.54140841960907 0.00117981503717601
1.63207948207855 0.000832417630590498
1.72275054454803 0.000605866895057261
1.81342160701752 0.000392965303035453
1.904092669487 0.000262558925896883
1.99476385116577 0.000176104615093209
2.08543491363525 0.000128036059322767
2.17610597610474 8.1946091086138e-05
2.26677703857422 5.93329095863737e-05
2.3574481010437 3.4680291719269e-05
2.44811916351318 2.10019788937643e-05
2.53879022598267 1.26186678244267e-05
2.62946128845215 7.88074339652667e-06
2.72013235092163 4.8504484766454e-06
2.81080365180969 2.49127629103896e-06
2.90147471427917 1.53988207785005e-06
2.99214577674866 9.36717356125882e-07
3.08281683921814 5.2214528523109e-07
3.17348790168762 3.10589456375965e-07
3.2641589641571 1.72542257814712e-07
3.35483002662659 8.50011758757319e-08
3.44550108909607 5.44816103342782e-08
3.53617215156555 2.82335630430453e-08
3.62684321403503 1.09987858820659e-08
3.71751427650452 5.85985659995458e-09
3.808185338974 3.13063464041363e-09
3.89885663986206 1.96687288678277e-09
3.98952770233154 9.04052999128879e-10
4.08019876480103 4.43834219376882e-10
4.17086982727051 1.87294540987537e-10
4.26154088973999 1.27070992617107e-10
4.35221195220947 5.73537710379934e-11
4.44288301467896 1.60940063359538e-11
};
\addplot [semithick, firebrick2022328]
table {%
0 1098.62524414062
0.0906710848212242 27.5796070098877
0.181342169642448 2.20185112953186
0.272013247013092 1.36714315414429
0.362684339284897 0.571439623832703
0.453355401754379 0.459119886159897
0.544026494026184 0.349796652793884
0.634697556495667 0.308272272348404
0.725368678569794 0.339260637760162
0.816039741039276 0.289992362260818
0.906710803508759 0.2967908680439
0.997381925582886 0.281587302684784
1.08805298805237 0.269043892621994
1.17872405052185 0.330730646848679
1.26939511299133 0.284455746412277
1.36006617546082 0.235984370112419
1.45073735713959 0.24878603219986
1.54140841960907 0.285902708768845
1.63207948207855 0.250260680913925
1.72275054454803 0.30636391043663
1.81342160701752 0.247209146618843
1.904092669487 0.281911075115204
1.99476385116577 0.288444817066193
2.08543491363525 0.252992630004883
2.17610597610474 0.249017432332039
2.26677703857422 0.27422684431076
2.3574481010437 0.256414920091629
2.44811916351318 0.274757295846939
2.53879022598267 0.23761822283268
2.62946128845215 0.247417077422142
2.72013235092163 0.258806616067886
2.81080365180969 0.289399445056915
2.90147471427917 0.270799547433853
2.99214577674866 0.268851190805435
3.08281683921814 0.247827798128128
3.17348790168762 0.243104487657547
3.2641589641571 0.250977605581284
3.35483002662659 0.282303899526596
3.44550108909607 0.260482251644135
3.53617215156555 0.251912623643875
3.62684321403503 0.235082238912582
3.71751427650452 0.270663410425186
3.808185338974 0.29893085360527
3.89885663986206 0.261995941400528
3.98952770233154 0.265284270048141
4.08019876480103 0.237848535180092
4.17086982727051 0.283851742744446
4.26154088973999 0.215535193681717
4.35221195220947 0.26943576335907
4.44288301467896 0.121421240270138
};
\addplot [semithick, steelblue32112180]
table {%
0 1126.67175292969
0.0906710848212242 25.6256637573242
0.181342169642448 1.7820188999176
0.272013247013092 0.932070910930634
0.362684339284897 0.23353023827076
0.453355401754379 0.104006417095661
0.544026494026184 0.0440454408526421
0.634697556495667 0.024686511605978
0.725368678569794 0.0123256305232644
0.816039741039276 0.0050859865732491
0.906710803508759 0.00383010134100914
0.997381925582886 0.00178420462179929
1.08805298805237 0.00100295234005898
1.17872405052185 0.000380984303774312
1.26939511299133 0.000185490120202303
1.36006617546082 8.04581650299951e-05
1.45073735713959 3.62546052201651e-05
1.54140841960907 1.49950392369647e-05
1.63207948207855 6.3802135628066e-06
1.72275054454803 2.65678158939409e-06
1.81342160701752 9.31763054268231e-07
1.904092669487 3.3885493166963e-07
1.99476385116577 1.17868630411522e-07
2.08543491363525 4.4168938728717e-08
2.17610597610474 1.36285915885992e-08
2.26677703857422 4.8296535659631e-09
2.3574481010437 1.30116006857861e-09
2.44811916351318 3.57083196345087e-10
2.53879022598267 9.36050958966206e-11
2.62946128845215 2.4939005721647e-11
2.72013235092163 6.33123588278384e-12
2.81080365180969 1.2935141239373e-12
2.90147471427917 3.15593769650499e-13
2.99214577674866 7.68717568441248e-14
3.08281683921814 2.80412798287378e-14
3.17348790168762 7.58428472883701e-15
3.2641589641571 3.73901391686787e-15
3.35483002662659 3.07273631824998e-15
3.44550108909607 3.45266786454322e-15
3.53617215156555 2.37200163109603e-15
3.62684321403503 2.43407432305319e-15
3.71751427650452 3.14379370043691e-15
3.808185338974 3.6770297398537e-15
3.89885663986206 3.73632924594155e-15
3.98952770233154 3.10376165280025e-15
4.08019876480103 3.0723780233133e-15
4.17086982727051 2.92187466814631e-15
4.26154088973999 1.47580667982485e-15
4.35221195220947 2.27841211372095e-15
4.44288301467896 8.91528265599927e-15
};
\addplot [semithick, crimson2385843]
table {%
0 1125.05847167969
0.0906710848212242 23.4622211456299
0.181342169642448 3.63257956504822
0.272013247013092 2.56079339981079
0.362684339284897 1.30488455295563
0.453355401754379 1.29662621021271
0.544026494026184 1.22522830963135
0.634697556495667 1.106729388237
0.725368678569794 1.07612550258636
0.816039741039276 0.96763950586319
0.906710803508759 0.991211771965027
0.997381925582886 1.05690109729767
1.08805298805237 1.04868924617767
1.17872405052185 1.04321599006653
1.26939511299133 1.03837883472443
1.36006617546082 0.816757142543793
1.45073735713959 1.0114221572876
1.54140841960907 1.11204218864441
1.63207948207855 1.018226146698
1.72275054454803 1.06638598442078
1.81342160701752 1.06221139431
1.904092669487 0.996275544166565
1.99476385116577 1.01619482040405
2.08543491363525 1.09964406490326
2.17610597610474 0.875039875507355
2.26677703857422 1.06421172618866
2.3574481010437 1.01105678081512
2.44811916351318 0.9766606092453
2.53879022598267 1.00140810012817
2.62946128845215 0.921353459358215
2.72013235092163 0.987269759178162
2.81080365180969 0.903959393501282
2.90147471427917 1.05604112148285
2.99214577674866 1.0294873714447
3.08281683921814 0.91097229719162
3.17348790168762 1.04888105392456
3.2641589641571 1.00143158435822
3.35483002662659 1.02337646484375
3.44550108909607 1.08488738536835
3.53617215156555 1.10680949687958
3.62684321403503 1.04248869419098
3.71751427650452 0.880059063434601
3.808185338974 0.83653599023819
3.89885663986206 0.985842704772949
3.98952770233154 0.960833251476288
4.08019876480103 1.2010577917099
4.17086982727051 0.967259705066681
4.26154088973999 1.13463294506073
4.35221195220947 1.12883496284485
4.44288301467896 1.16157412528992
};
\addplot [semithick, steelblue65145197]
table {%
0 1126.37463378906
0.0906710848212242 24.8372688293457
0.181342169642448 1.45060253143311
0.272013247013092 0.619908690452576
0.362684339284897 0.110277660191059
0.453355401754379 0.0304753929376602
0.544026494026184 0.00766012258827686
0.634697556495667 0.00220596767030656
0.725368678569794 0.000534694117959589
0.816039741039276 9.22052349778824e-05
0.906710803508759 3.01974978356156e-05
0.997381925582886 4.96857364851166e-06
1.08805298805237 8.97407062439015e-07
1.17872405052185 9.99940539259114e-08
1.26939511299133 1.28787265296637e-08
1.36006617546082 1.31613397957864e-09
1.45073735713959 1.28497004703299e-10
1.54140841960907 1.06031381591487e-11
1.63207948207855 8.5543681513367e-13
1.72275054454803 6.49243842281572e-14
1.81342160701752 8.48851272882171e-15
1.904092669487 6.1355445633252e-15
1.99476385116577 7.50380728148543e-15
2.08543491363525 6.23156633580832e-15
2.17610597610474 3.83301720983768e-15
2.26677703857422 5.44492937879209e-15
2.3574481010437 9.19033542979642e-15
2.44811916351318 6.42205345773397e-15
2.53879022598267 5.91176650547361e-15
2.62946128845215 5.84461330989882e-15
2.72013235092163 4.25085390403702e-15
2.81080365180969 6.12699249517325e-15
2.90147471427917 5.47696416485725e-15
2.99214577674866 5.83393095388452e-15
3.08281683921814 9.5035258620437e-15
3.17348790168762 5.52010058824559e-15
3.2641589641571 3.20923843055709e-15
3.35483002662659 3.27903225134495e-15
3.44550108909607 3.01421460016595e-15
3.53617215156555 3.56667405232067e-15
3.62684321403503 3.51255224688115e-15
3.71751427650452 2.1520525856825e-15
3.808185338974 2.34130261598869e-15
3.89885663986206 2.89486702262311e-15
3.98952770233154 2.10931998525176e-15
4.08019876480103 2.44820071503102e-15
4.17086982727051 4.0949248793264e-15
4.26154088973999 1.92587064832661e-15
4.35221195220947 2.69928478576148e-15
4.44288301467896 1.69777198129019e-15
};
\addplot [semithick, tomato25010573]
table {%
0 1070.54223632812
0.0906710848212242 33.1056976318359
0.181342169642448 5.54709053039551
0.272013247013092 3.0888888835907
0.362684339284897 2.60351014137268
0.453355401754379 2.88509583473206
0.544026494026184 2.39535236358643
0.634697556495667 2.90875315666199
0.725368678569794 2.75224900245667
0.816039741039276 3.45414710044861
0.906710803508759 3.12077450752258
0.997381925582886 2.66711211204529
1.08805298805237 2.78555011749268
1.17872405052185 3.15317416191101
1.26939511299133 3.39944410324097
1.36006617546082 2.69769787788391
1.45073735713959 3.01088857650757
1.54140841960907 2.95125412940979
1.63207948207855 3.14198875427246
1.72275054454803 3.00300407409668
1.81342160701752 3.00213003158569
1.904092669487 3.25444412231445
1.99476385116577 3.11526656150818
2.08543491363525 2.95249652862549
2.17610597610474 2.94375228881836
2.26677703857422 2.84272885322571
2.3574481010437 3.4002206325531
2.44811916351318 2.9451425075531
2.53879022598267 2.97072839736938
2.62946128845215 3.13289356231689
2.72013235092163 2.63815593719482
2.81080365180969 2.72272515296936
2.90147471427917 2.8491427898407
2.99214577674866 2.94208955764771
3.08281683921814 2.81294822692871
3.17348790168762 2.84282326698303
3.2641589641571 3.02081227302551
3.35483002662659 2.7052800655365
3.44550108909607 2.61668252944946
3.53617215156555 2.75383973121643
3.62684321403503 3.25029850006104
3.71751427650452 2.88732767105103
3.808185338974 2.98327302932739
3.89885663986206 3.84475040435791
3.98952770233154 3.28820157051086
4.08019876480103 2.96359276771545
4.17086982727051 3.04488277435303
4.26154088973999 3.6370964050293
4.35221195220947 3.82412981987
4.44288301467896 1.54687511920929
};
\addplot [semithick, cornflowerblue106173213]
table {%
0 1125.40991210938
0.0906710848212242 22.5008335113525
0.181342169642448 0.751912534236908
0.272013247013092 0.167893797159195
0.362684339284897 0.010254523716867
0.453355401754379 0.000609229726251215
0.544026494026184 2.97303558909334e-05
0.634697556495667 1.02585556760459e-06
0.725368678569794 2.33733921106705e-08
0.816039741039276 2.54072318739418e-10
0.906710803508759 5.81764107374094e-12
0.997381925582886 5.03466964841583e-14
1.08805298805237 4.66070688919201e-15
1.17872405052185 9.13520120822669e-15
1.26939511299133 5.99896515926165e-15
1.36006617546082 8.14868311038329e-15
1.45073735713959 8.44755783878902e-15
1.54140841960907 6.72399613947466e-15
1.63207948207855 8.48884730683588e-15
1.72275054454803 7.12657946435984e-15
1.81342160701752 7.826194797474e-15
1.904092669487 3.99226745073449e-15
1.99476385116577 8.52255837110365e-15
2.08543491363525 5.21736296608391e-15
2.17610597610474 7.32955905170807e-15
2.26677703857422 4.2952824761864e-15
2.3574481010437 7.89427507060956e-15
2.44811916351318 5.84080166163617e-15
2.53879022598267 5.65437987434087e-15
2.62946128845215 4.62917312311515e-15
2.72013235092163 4.25580438809725e-15
2.81080365180969 6.21983958817005e-15
2.90147471427917 4.21142706144117e-15
2.99214577674866 5.35618743097415e-15
3.08281683921814 1.01863157326936e-14
3.17348790168762 3.86951416546898e-15
3.2641589641571 3.61474444262678e-15
3.35483002662659 2.40162131447032e-15
3.44550108909607 2.70077450495747e-15
3.53617215156555 2.86417541905406e-15
3.62684321403503 2.59522657643306e-15
3.71751427650452 3.16019141126281e-15
3.808185338974 3.25519399135214e-15
3.89885663986206 3.09507681223382e-15
3.98952770233154 1.68488469263507e-15
4.08019876480103 1.82977793683416e-15
4.17086982727051 2.33976715701355e-15
4.26154088973999 1.75458332809549e-15
4.35221195220947 2.47945030155408e-15
4.44288301467896 1.3813929993921e-15
};
\addplot [semithick, salmon251145113]
table {%
0 945.397521972656
0.0906710848212242 40.1411170959473
0.181342169642448 10.5644683837891
0.272013247013092 7.83350133895874
0.362684339284897 7.15244626998901
0.453355401754379 7.42622137069702
0.544026494026184 7.90521049499512
0.634697556495667 7.86223936080933
0.725368678569794 8.34747791290283
0.816039741039276 7.66156768798828
0.906710803508759 8.27422332763672
0.997381925582886 7.83301639556885
1.08805298805237 7.7625937461853
1.17872405052185 6.78865528106689
1.26939511299133 8.49681854248047
1.36006617546082 6.68622589111328
1.45073735713959 7.66005802154541
1.54140841960907 7.75427293777466
1.63207948207855 8.41468524932861
1.72275054454803 7.48938131332397
1.81342160701752 7.39064979553223
1.904092669487 7.4653787612915
1.99476385116577 7.97520732879639
2.08543491363525 7.18162822723389
2.17610597610474 7.53485727310181
2.26677703857422 7.31877708435059
2.3574481010437 6.96071767807007
2.44811916351318 7.38452816009521
2.53879022598267 7.57715511322021
2.62946128845215 7.16027021408081
2.72013235092163 7.315101146698
2.81080365180969 7.63667964935303
2.90147471427917 7.49803590774536
2.99214577674866 7.97885799407959
3.08281683921814 6.91310834884644
3.17348790168762 7.47106075286865
3.2641589641571 6.99009227752686
3.35483002662659 7.73245191574097
3.44550108909607 7.90038824081421
3.53617215156555 6.55440425872803
3.62684321403503 7.19968509674072
3.71751427650452 6.62579917907715
3.808185338974 7.55898380279541
3.89885663986206 6.75478935241699
3.98952770233154 8.98880577087402
4.08019876480103 6.82914686203003
4.17086982727051 8.38577461242676
4.26154088973999 7.09687519073486
4.35221195220947 4.84073448181152
4.44288301467896 7.940758228302
};
\addplot [semithick, lightsteelblue157201224]
table {%
0 1122.34802246094
0.0906710848212242 16.8305530548096
0.181342169642448 0.102657318115234
0.272013247013092 0.00304131698794663
0.362684339284897 7.23166476745973e-06
0.453355401754379 3.6920937418472e-09
0.544026494026184 1.16038342129476e-12
0.634697556495667 1.2519075809651e-14
0.725368678569794 4.57166593874369e-15
0.816039741039276 7.10138235176139e-15
0.906710803508759 5.40764934120106e-15
0.997381925582886 9.10158585868195e-15
1.08805298805237 5.87015812952211e-15
1.17872405052185 1.15194846052997e-14
1.26939511299133 5.39963429193767e-15
1.36006617546082 1.00878803398273e-14
1.45073735713959 5.08980022774388e-15
1.54140841960907 2.84681607172314e-14
1.63207948207855 5.81998921508919e-15
1.72275054454803 7.17523557794897e-15
1.81342160701752 6.33727435355976e-15
1.904092669487 4.69900294280327e-15
1.99476385116577 8.43802871813241e-15
2.08543491363525 6.56118920723233e-15
2.17610597610474 9.00904242699674e-15
2.26677703857422 4.8014592010702e-15
2.3574481010437 1.03904743899044e-14
2.44811916351318 3.75764228896036e-15
2.53879022598267 5.01336439810013e-15
2.62946128845215 3.5490305677876e-15
2.72013235092163 4.30526518298627e-15
2.81080365180969 3.66648121504507e-15
2.90147471427917 6.2755709679676e-15
2.99214577674866 5.7196937378707e-15
3.08281683921814 1.13109323881914e-14
3.17348790168762 3.04892579858619e-15
3.2641589641571 2.08372370837692e-15
3.35483002662659 2.09143043764751e-15
3.44550108909607 2.19940808018112e-15
3.53617215156555 2.61068852761047e-15
3.62684321403503 2.78769723776294e-15
3.71751427650452 2.31468079397296e-15
3.808185338974 2.34243488728093e-15
3.89885663986206 2.59051199104864e-15
3.98952770233154 2.05208448669813e-15
4.08019876480103 3.02837508521991e-15
4.17086982727051 1.94494307744169e-15
4.26154088973999 1.48467829115615e-15
4.35221195220947 2.67849563262055e-15
4.44288301467896 1.26295989979493e-15
};
\addplot [semithick, lightpink252186160]
table {%
0 1145.59143066406
0.0906710848212242 57.7472686767578
0.181342169642448 14.2994861602783
0.272013247013092 19.7445182800293
0.362684339284897 19.4584407806396
0.453355401754379 16.7837467193604
0.544026494026184 16.233736038208
0.634697556495667 17.6969108581543
0.725368678569794 16.8014850616455
0.816039741039276 16.3008327484131
0.906710803508759 16.9415130615234
0.997381925582886 19.351842880249
1.08805298805237 17.5870990753174
1.17872405052185 18.4037246704102
1.26939511299133 16.014217376709
1.36006617546082 16.1167335510254
1.45073735713959 18.4115505218506
1.54140841960907 17.8528633117676
1.63207948207855 18.8805751800537
1.72275054454803 17.1256122589111
1.81342160701752 17.6611843109131
1.904092669487 16.6902599334717
1.99476385116577 17.9808464050293
2.08543491363525 16.9603881835938
2.17610597610474 15.9144887924194
2.26677703857422 15.8522529602051
2.3574481010437 17.3269386291504
2.44811916351318 18.040599822998
2.53879022598267 17.910285949707
2.62946128845215 16.4636936187744
2.72013235092163 17.5221252441406
2.81080365180969 17.9425792694092
2.90147471427917 16.9594631195068
2.99214577674866 16.8636684417725
3.08281683921814 17.9369239807129
3.17348790168762 15.4929132461548
3.2641589641571 18.0834121704102
3.35483002662659 16.3559741973877
3.44550108909607 16.7217979431152
3.53617215156555 17.6654396057129
3.62684321403503 16.2088775634766
3.71751427650452 16.3369159698486
3.808185338974 16.9791278839111
3.89885663986206 16.5943717956543
3.98952770233154 15.5593099594116
4.08019876480103 14.6236763000488
4.17086982727051 17.5485401153564
4.26154088973999 21.0737705230713
4.35221195220947 12.9009237289429
4.44288301467896 30.2852325439453
};
\addplot [semithick, powderblue197218238]
table {%
0 1113.32934570312
0.0906710848212242 7.97391986846924
0.181342169642448 0.000385360704967752
0.272013247013092 2.02206376087588e-08
0.362684339284897 2.25771160257794e-14
0.453355401754379 1.69967613253144e-14
0.544026494026184 5.92723840928816e-15
0.634697556495667 6.77532464201237e-15
0.725368678569794 6.91284594671326e-15
0.816039741039276 1.41702200036234e-14
0.906710803508759 6.7489925052646e-15
0.997381925582886 5.99581758482966e-15
1.08805298805237 2.11253892220956e-15
1.17872405052185 6.66856672692281e-15
1.26939511299133 4.5186332059161e-15
1.36006617546082 8.35123240499431e-15
1.45073735713959 6.60654993914016e-15
1.54140841960907 4.68819988459399e-15
1.63207948207855 5.32957069115611e-15
1.72275054454803 8.60779529658585e-15
1.81342160701752 6.04802361350073e-15
1.904092669487 4.07647141953751e-15
1.99476385116577 4.27810634208198e-15
2.08543491363525 3.63479752413655e-15
2.17610597610474 3.52267704345792e-15
2.26677703857422 3.00782648943599e-15
2.3574481010437 1.44328332515571e-14
2.44811916351318 3.85621236006529e-15
2.53879022598267 5.71611205905324e-15
2.62946128845215 4.01529361788912e-15
2.72013235092163 2.9012777914844e-15
2.81080365180969 6.29378471743241e-15
2.90147471427917 3.05738088146568e-15
2.99214577674866 7.24519457016154e-15
3.08281683921814 5.82037546211314e-15
3.17348790168762 2.32787375564292e-15
3.2641589641571 2.82639224389236e-15
3.35483002662659 1.9806520806738e-15
3.44550108909607 2.24640803260013e-15
3.53617215156555 1.79195982156339e-15
3.62684321403503 2.02195023080837e-15
3.71751427650452 1.75866539162654e-15
3.808185338974 1.58944578469879e-15
3.89885663986206 1.76502057395067e-15
3.98952770233154 1.43147890459619e-15
4.08019876480103 1.84843870793688e-15
4.17086982727051 1.79120469169091e-15
4.26154088973999 1.74052215765459e-15
4.35221195220947 2.40799735498078e-15
4.44288301467896 2.12568847344097e-15
};
\addplot [semithick, blanchedalmond253223209]
table {%
0 1091.91516113281
0.0906710848212242 74.6991729736328
0.181342169642448 30.0098552703857
0.272013247013092 24.7565364837646
0.362684339284897 35.5260887145996
0.453355401754379 31.6102313995361
0.544026494026184 41.7357292175293
0.634697556495667 37.9227409362793
0.725368678569794 37.8751983642578
0.816039741039276 32.601203918457
0.906710803508759 31.9273586273193
0.997381925582886 36.7572479248047
1.08805298805237 37.7310104370117
1.17872405052185 32.5780906677246
1.26939511299133 31.640905380249
1.36006617546082 32.9426879882812
1.45073735713959 37.3659934997559
1.54140841960907 32.1462898254395
1.63207948207855 34.9634132385254
1.72275054454803 34.7719688415527
1.81342160701752 32.3448524475098
1.904092669487 32.6706657409668
1.99476385116577 36.6783027648926
2.08543491363525 34.3338432312012
2.17610597610474 34.601318359375
2.26677703857422 35.306324005127
2.3574481010437 33.9546928405762
2.44811916351318 33.248592376709
2.53879022598267 32.9114723205566
2.62946128845215 32.9185104370117
2.72013235092163 33.3576889038086
2.81080365180969 34.8956832885742
2.90147471427917 35.0721015930176
2.99214577674866 32.2315864562988
3.08281683921814 32.8855094909668
3.17348790168762 35.6764221191406
3.2641589641571 35.3247985839844
3.35483002662659 34.184741973877
3.44550108909607 33.9815139770508
3.53617215156555 34.6205253601074
3.62684321403503 33.344181060791
3.71751427650452 35.2783432006836
3.808185338974 30.2657604217529
3.89885663986206 28.759256362915
3.98952770233154 31.9429588317871
4.08019876480103 38.2185554504395
4.17086982727051 27.8541469573975
4.26154088973999 31.4215335845947
4.35221195220947 34.8802299499512
4.44288301467896 11.4002962112427
};
\addplot [semithick, lavender221234246]
table {%
0 1092.2099609375
0.0906710848212242 1.18654155731201
0.181342169642448 5.31658432556537e-11
0.272013247013092 6.72004388374277e-15
0.362684339284897 1.34267393752698e-13
0.453355401754379 5.28727155983612e-15
0.544026494026184 7.62746900958688e-15
0.634697556495667 6.71923454376167e-15
0.725368678569794 1.68507870553164e-14
0.816039741039276 4.83976025217586e-14
0.906710803508759 5.84474460000564e-15
0.997381925582886 2.63023347405519e-14
1.08805298805237 5.2611956505549e-15
1.17872405052185 8.70271634975401e-15
1.26939511299133 4.44511667532506e-15
1.36006617546082 6.30233466800199e-15
1.45073735713959 3.50958170233513e-15
1.54140841960907 2.42107647542263e-14
1.63207948207855 3.36670566709993e-15
1.72275054454803 2.85430028543849e-15
1.81342160701752 3.71112239246421e-15
1.904092669487 5.14752467606632e-15
1.99476385116577 3.60625463139645e-15
2.08543491363525 4.64325504586326e-15
2.17610597610474 5.25948167938613e-15
2.26677703857422 3.47263836034063e-15
2.3574481010437 2.09221542543138e-14
2.44811916351318 2.6605819445773e-15
2.53879022598267 5.10800550687922e-15
2.62946128845215 2.59622014608019e-15
2.72013235092163 1.89879735774999e-15
2.81080365180969 5.68794143729345e-15
2.90147471427917 5.27181574964757e-15
2.99214577674866 4.28710903176187e-15
3.08281683921814 2.2118579821981e-15
3.17348790168762 3.11212991480265e-15
3.2641589641571 2.29368665885879e-15
3.35483002662659 1.83816970400084e-15
3.44550108909607 1.5761192035814e-15
3.53617215156555 2.16845093178311e-15
3.62684321403503 1.70845772543628e-15
3.71751427650452 1.37473616745962e-15
3.808185338974 1.68761235048347e-15
3.89885663986206 1.9147982336401e-15
3.98952770233154 1.38656159443624e-15
4.08019876480103 1.76152497485647e-15
4.17086982727051 1.57138778341716e-15
4.26154088973999 1.59109305202296e-15
4.35221195220947 1.64404055216024e-15
4.44288301467896 1.27196576584838e-15
};
\addplot [thick, black]
table {%
0 1126.80261230469
0.0906710848212242 25.9837036132812
0.181342169642448 1.95186972618103
0.272013247013092 1.11620664596558
0.362684339284897 0.32591837644577
0.453355401754379 0.179122000932693
0.544026494026184 0.0956870913505554
0.634697556495667 0.0720205679535866
0.725368678569794 0.0494311302900314
0.816039741039276 0.0299995001405478
0.906710803508759 0.0328643806278706
0.997381925582886 0.0242792814970016
1.08805298805237 0.0224402267485857
1.17872405052185 0.0147643256932497
1.26939511299133 0.0129452524706721
1.36006617546082 0.0106458496302366
1.45073735713959 0.00944889523088932
1.54140841960907 0.0080562736839056
1.63207948207855 0.00709288101643324
1.72275054454803 0.00659846188500524
1.81342160701752 0.00560837471857667
1.904092669487 0.00489904405549169
1.99476385116577 0.0043848087079823
2.08543491363525 0.00427129445597529
2.17610597610474 0.00376165565103292
2.26677703857422 0.00373295182362199
2.3574481010437 0.00307339802384377
2.44811916351318 0.00263112550601363
2.53879022598267 0.00227850279770792
2.62946128845215 0.00207001506350935
2.72013235092163 0.00188188150059432
2.81080365180969 0.00145697756670415
2.90147471427917 0.00135578867048025
2.99214577674866 0.00129466212820262
3.08281683921814 0.0011107447789982
3.17348790168762 0.00101656408514827
3.2641589641571 0.000906687520910054
3.35483002662659 0.00074621953535825
3.44550108909607 0.000786912976764143
3.53617215156555 0.000678830256219953
3.62684321403503 0.000439566996647045
3.71751427650452 0.000399994372855872
3.808185338974 0.000370423193089664
3.89885663986206 0.000409886328270659
3.98952770233154 0.000338785612257197
4.08019876480103 0.000305637338897213
4.17086982727051 0.000222609785851091
4.26154088973999 0.000306488189380616
4.35221195220947 0.000232086182222702
4.44288301467896 0.000108207059383858
};
\end{axis}

